Revisiting the Mazur bound and the Suzuki equality

Among the few known rigorous results for time-dependent equilibrium correlations, important for understanding transport properties, are the Mazur bound and the Suzuki equality. The Mazur inequality gives a lower bound, on the long-time average of the time-dependent auto-correlation function of observables, in terms of equilibrium correlation functions involving conserved quantities. On the other hand, Suzuki proposes an exact equality for quantum systems. In this paper, we discuss the relation between the two results and in particular, look for the analogue of the Suzuki result for classical systems. This requires us to examine as to what constitutes a complete set of conserved quantities required to saturate the Mazur bound. We present analytic arguments as well as illustrative numerical results from a number of different systems. Our examples include systems with few degrees of freedom as well as many-particle integrable models, both free and interacting.

==> macros.tex <==

\newcommand{\nb}{{\em n.b.}}
\newcommand{\eg}{{\em e.g.}}
\newcommand\ie{i.e. }

\newcommand\etal{et al.}
\newcommand{\lref}[2][]{\hyperref[#2]{#1~\ref*{#2}}}
\renewcommand{\eqref}[1]{\hyperref[#1]{(\ref*{#1})}}
\def\abs#1{\left| #1 \right|}




\newcommand{\TwoToOne}{2-to-1}
\renewcommand{\cal}{\mathcal}
\numberwithin{equation}{section}


% CUSTOM COMMANDS
\newcommand{\angstrom}{\text{\normalfont\AA}}
\newcommand{\braket}[3]{\bra{#1}\;#2\;\ket{#3}}
\newcommand{\projop}[2]{ \ket{#1}\bra{#2}}
%\newcommand{\ket}[1]{ \vrule\;#1\;\rangle}
\newcommand{\ket}[1]{ |\;#1\;\rangle}
%\newcommand{\bra}[1]{ \langle\;#1\;\vrule}
\newcommand{\bra}[1]{ \langle\;#1\;|}
\newcommand{\iprod}[2]{ \langle#1|#2\rangle}
\newcommand{\intl}[2]{\int\limits_{#1}^{#2}}
\newcommand{\logt}[1]{\log_2\left(#1\right)}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\mf}[1]{\mathbf{#1}}

\newcommand{\cx}[1]{\tilde{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\p}{\partial}
\newcommand{\cmnt}[2]{\textbf{}{\color{#1}#2}\textbf{}}
\newcommand{\hx}[1]{\hat{#1}}

%\newcommand{\flap}{\mb{L}}
%\newcommand{\fcurr}{\mb{A}}
%\newcommand{\flapFull}{|\Delta|^{3/4}}
%\newcommand{\tdir}{f}
%\newcommand{\mzeta}{\zeta}
%newcommand{\implies}{\Longleftrightarrow}%for not using amsmath
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}

\newcommand{\eqa}[1]{\begin{align}#1\end{align}}%amsmath
%\newcommand{\eqa}[1]{\begin{eqnarray} #1\end{eqnarray}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\iu}{{i\mkern1mu}}
\newcommand{\widesim}[2][1.5]{
	\mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}
}

\newcommand{\sina}{\alpha}
\newcommand{\HTheta}{\theta}
\newcommand{\genpower}{\beta}
\newcommand{\cosa}{\phi}
\newcommand{\RN}[1]{%ROMAN NUMBER CONVERTER
	\textup{\uppercase\expandafter{\romannumeral#1}}%
}
	
%BS model

\usepackage{color}
\definecolor{dgreen}{rgb}{0,0.7,0}
\def\redw#1{{\color{black} #1}}
\def\greenw#1{{\color{dgreen} #1}}
\def\bluew#1{{\color{blue} #1}}

\usepackage{url,hyperref}

%\usepackage{caption}
%\usepackage{subcaption}

\newcommand{\dd}{\mathrm{d}}

\newcommand{\ci}{\mathrm{i}}
\newcommand{\Erfc}{\mathrm{Erfc}}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\Erf}{\mathrm{Erf}}
\newcommand{\Erfi}{\mathrm{Erfi}}
\newcommand{\Ei}{\mathrm{Ei}}
\newcommand{\gammae}{\gamma_\mathrm{E}}

\newcommand{\rhobar}{\overline{\rho}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cY}{\mathcal{Y}_a}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cC}{\mathcal{C}_a}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cV}{\mathcal{V}_a}


\newcommand{\cCinf}{{\cC_\infty}}

\newcommand{\zt}{\tilde{z}}
\newcommand{\zh}{\hat{z}}
\newcommand{\tfG}{\mathfrak{G}}

\newcommand{\br}{\mathbf{r}}
\newcommand{\brz}{\mathbf{r}_0}
\newcommand{\bk}{\mathbf{k}}

\newcommand{\omegain}{\omega_{in}}
\newcommand{\omegatyp}{\overline{\omega}}
\newcommand{\jtyp}{j^0}
\newcommand{\jopt}{j^s}
\newcommand{\Haux}{\mathcal{T}_r}
\newcommand{\omegast}{\omega^*}
\newcommand{\hst}{h^*}
\newcommand{\of}{\overline{f}}

\newcommand{\bG}{G_{ss}}


%Fractional BS
\usepackage{verbatim}
%\usetikzlibrary{arrows,shapes}
\usepackage{graphicx,epstopdf}  % needed for figures

\usepackage{amsfonts}
\usepackage{color}
\usepackage{dcolumn}   % needed for some tables
\usepackage{bm}        % for math
\usepackage{amssymb}   % for math
\usepackage{hyperref}
\usepackage{dcolumn}   % needed for some tables
\usepackage{bm} 
\usepackage{amssymb}  
\usepackage{verbatim}
\usepackage{breqn}
\usepackage{array}
\usepackage{enumerate}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bed{\begin{dmath*}}
	\def\eed{\end{dmath*}}

%	\newcommand{\angstrom}{\text{\nnrmalfont\AA}}
%\newcommand{\braket}[3]{\bra{#1}\;#2\;\ket{#3}}
%\newcommand{\projop}[2]{ \ket{#1}\bra{#2}}
%\newcommand{\ket}[1]{ \vrule\;#1\;\rangle}
%\newcommand{\ket}[1]{ |\;#1\;\rangle}
%\newcommand{\bra}[1]{ \langle\;#1\;\vrule}
%\newcommand{\bra}[1]{ \langle\;#1\;|}
%\newcommand{\iprod}[2]{ \langle\;#1\;|\;#2\;\rangle}
%\newcommand{\intl}[2]{\int\limits_{#1}^{#2}}
%\newcommand{\logt}[1]{\log_2\left(#1\right)}
\def\cI{\mathcal{I}}
%\newcommand{\mb}[1]{\mathbb{#1}}
%\newcommand{\cx}[1]{\tilde{#1}}
\newcommand{\dx}[1]{\hat{#1}}
%\newcommand{\nn}{\nonumber}
%\newcommand{\la}{\langle}
%\newcommand{\ra}{\rangle}
%\newcommand{\p}{\partial}
%\newcommand{\cmnt}[2]{\textbf{\#\#}{\color{#1}#2}\textbf{\#\#}}
%\newcommand{\mc}[1]{\mathcal{#1}}
%\newcommand{\flap}{\mb{L}}
%\newcommand{\flapFull}{|\Delta|^{3/4}}
%\newcommand{\tdir}{v}
%\newcommand{\mzeta}{\zeta}


%Frac Laplacian HCME

%\newcommand{\sina}{\alpha}
%\newcommand{\HTheta}{\theta}
%\newcommand{\genpower}{\beta}
%\newcommand{\cosa}{\phi}
	\newcommand{\flap}{\mb{L}_{\bar{\kappa}}}
\newcommand{\flapfinite}{\mb{L}}
\newcommand{\fcurr}{\mb{A}}
\newcommand{\flapFull}{|\Delta|^{3/4}}
\newcommand{\tdir}{f}
\newcommand{\mzeta}{\zeta}
\newcommand{\momsym}{\delta}

	\newcommand{\blang}{\big \langle}
\newcommand{\brang}{\big \rangle}
